Towards Full-to-Empty Room Generation with Structure-Aware Feature Encoding and Soft Semantic Region-Adaptive Normalization

The task of transforming a furnished room image into a background-only is extremely challenging since it requires making large changes regarding the scene context while still preserving the overall layout and style. In order to acquire photo-realistic and structural consistent background, existing deep learning methods either employ image inpainting approaches or incorporate the learning of the scene layout as an individual task and leverage it later in a not fully differentiable semantic region-adaptive normalization module. To tackle these drawbacks, we treat scene layout generation as a feature linear transformation problem and propose a simple yet effective adjusted fully differentiable soft semantic region-adaptive normalization module (softSEAN) block. We showcase the applicability in diminished reality and depth estimation tasks, where our approach besides the advantages of mitigating training complexity and non-differentiability issues, surpasses the compared methods both quantitatively and qualitatively. Our softSEAN block can be used as a drop-in module for existing discriminative and generative models. Implementation is available on vcl3d.github.io/PanoDR/.

==> Application.tex <==

\begin{comment}
\begin{enumerate}
    \item Show AR on top of DR
    \item use segmentation masks to composite original / other object within the mask? (to avoid 3d rendering)
    \item needs nice (colored) alpha blending effect for AR
    \item diminishing multiple objects simultaneously
\end{enumerate}
\end{comment}

==> Dataset.tex <==
\input{figures/dataset}

While there exists a variety of datasets of indoor scenes like Matterport3D \cite{chang2018matterport3d} and Stanford2D3D \cite{armeni2017joint}, also including spherical panoramas, they are not suitable for DR.
The task that we tackle in this work is fundamentally different from all the previously explored methods for the simple reason that removing an object from an image must be supervised with the occluded content.

Therefore, we employ the Structured3D dataset \cite{Structured3D}, which provides, among others, photo-realistic spherical panoramas of indoor scenes with 3 different configurations (\textit{empty, simple, and full room}), accompanied by layout and semantic label annotations, making it highly suitable for DR object removal.
Considering a normalized indoor scene color image $\im_f \in \mathbb{R}^{W \times H \times 3} \, \, | \, \, 0 \leq \im_f(\mathbf{p}) \leq 1$, with $\mathbf{p} \in \Omega$, and $\Omega$ being the image domain of width $W$ and height $H = \frac{W}{2}$, which corresponds to either the simple or full configuration of Structured3D, we seek to remove a foreground object by replacing its appearance with the occluded background.
The latter corresponds to the matching scene empty image $\im_b$, which contains a minimal, structure only, WCF (wall--ceiling--floor) representation of the same scene.
In addition, Structured3D offers the scene layout's junction positions, which after projecting the connected wireframe reconstruction on the panorama, provide a dense layout WCF segmentation $\layout \in \mathbb{N}^{W \times H}$ of the $\im_{f/b}$ scene, with $\layout(\mathbf{p}) \in \{ 1, 2, 3 \}$.

To learn the removal of objects, we additionally exploit the semantic labeling of each scene.
We randomly pick the largest connected component of one of the available foreground classes as the input object mask $\obj$ denoting the region to be diminished.
The mask $\obj$ is a binary mask with ones in the diminished region and zeros elsewhere, while $\bar{\obj}$ is its binary inverse mask.
Since the masks are pixel perfect, we calculate their convex to simulate a generic, convex polygon region selection. 
This way, we can supervise the DR task for the diminishing of an input image $\im_f$ at the region denoted by $\obj$, using the background image $\im_b$.
However, this straightforward way fails in practice because of conflicting supervision signals.
Structured3D is photorealistically rendered using physically based ray-tracing.
As a result, the inclusion of foreground introduces light ray bounces, and more importantly, the lights themselves, which are added into the scene as new foreground objects participate into the new image formation process, creating a photo-inconsistency between $\im_f$ and $\im_b$.
To overcome this issue, we perform reverse compositing of selected foreground object classes (\textit{i.e.}~excluding lights) into the background.
While this is not a perfect solution as incident shadows are lost, it allows for proper training that is not hindered by irregular supervision across the training samples.
An illustrative example of this process and the defects it solves is presented in Figure~\ref{fig:dataset}.

\begin{comment}
While image completion is among the top trends in the computer vision research, their approach is well formulated. 
More precisely, the paradigm of the dataset samples is to generate predefined shape masks \textbf{MAYBE SOME REFERENCES} or to create free form ones \textbf{REFERENCES ASWELL}, corrupting the image with the aforementioned mask and supervising the learning procedure with the original image.
The task that we tackle in this work is fundamentally different from all the previously explored methods for the simple reason that removing an object from an image must be supervised with empty space.
To this end we employ the synthetic dataset of \cite{Structured3D}, which provides, among others, photo-realistic indoor panoramic images of the same room with 3 different decorations (\textit{empty room, simple room, full room}), accompanied by 3D, layout and semantic annotations, enabling deep-learning research for Diminished Reality \textbf{CHECK COHERENCY} applications. 
Since our work has Diminished Reality application flavor, we produce object masks as convex hulls (see fig\ref{fig:dataset}a) of the selected-to-remove objects, to cover a generic variety of shapes\textbf{EDW THELEI KALUTERO JUSTIFICATION}. 
More precisely, at the training stage we select an object from the semantic map to remove at random and compute the convex hull of the pixel-perfect mask. 
While this work for the most of the rooms, there are rooms that have only tiny objects, or being not decorated, leading to the computation of tiny masks or no masks at all.
For the sake of training efficiency  we want to avoid to remove tiny masks  \textbf{NEED HELP}, so we handle both samples by creating a random rectangular mask (with predefined size range).
A straightforward approach for dealing with Diminished Reality task would be to supervise a masked full room sample with the corresponding empty one. 
In theory this is a valid reasoning, in practice it fails for the simple reason that this dataset is rendered using ray-tracing \textbf{DO WE NEED REF?}, which produces photo-realistic lighting and shading, which differs in the empty and non-empty rooms (see fig\ref{fig:dataset}b). 
To deal with this inconsistency,create samples by copying all the objects from the full room to the empty one, and supervising the task with the empty sample (see fig\ref{fig:dataset}c).
At last, our structural prior map is created by using the room corners data provided by the dataset.
We use the corners to create the ceiling-walls and the walls-floor junctions, which segments the room image in 3 segments (\textit{(ceiling, wall floor)} see fig\ref{fig:dataset}d) 
\end{comment}

\iffalse
We train our models using the, recently proposed, synthetic dataset of \cite{Structured3D}.
This dataset offers a variety of photo-realistic images of indoor scenes, created by professional interior designers and decorators, accompanied by rich 3D structure annotations as well as various objects configurations for each room (\textit{i.e.}~empty room, simple room and full room). 
Combining the multiple objects configurations with the dense semantic map for each room (which is included in the dataset), enables the possibility of composing an object oriented dataset suitable for DR. 
While replacing the pixels corresponding to an object in the full configuration with the corresponding ones from the empty configuration would be an good enough initial solution, in many cases it lacks of photo-realism due to the dataset generation using ray-tracing, which led to the different objects configurations having a slight color discrepancy created by reflective (floor tiles) or diffusive (curtains) materials in the scene. 
In order to overcome this, we approach the dataset generation in an additive rather than reductive manner. 
We augment the empty room configurations with all the objects from the full room configuration except the one we want to remove, which creates backgrounds with no color discrepancies with the remaining room. 
While composing the dataset samples in such way overcomes the color discrepancy issues, it produces less photo-realistic samples due to the lack of shadows. 
In order to generate the inpainting region masks, the convex hull of an object's pixel-perfect mask is computed, which we believe is the best compromise between pixel-perfect masks (not viable option for DR applications) and bounding boxes (which, in some cases, can be big relative to the object size). 
At last, our structural prior map is created by using the room corners data provided by the dataset.
We use the corners to create the ceiling-walls and the walls-floor junctions, which segments the room image in 3 segments (\textit{ceiling, wall floor}) \textbf{ADD FIGURE AND REFERENCE IT IN THE TEXT}.
%\begin{enumerate}
%    \item Structure3D full / empty
%    \item lighting issues
%    \item compositing solution
%\end{enumerate}
\fi

==> Layout.tex <==
A core module of our approach is the estimation of the room layout, which later with drive the hallucination of realistic samples. To this end we employ the well established \textbf{UNet} architecture originally proposed in \cite{ronneberger2015u}. The network consists of 4 down-sampling and up-sampling convolutional modules (refer to \ref{fig:networks}) for the detailed architecture. \textbf{EDW THA DWSW KAI KAPOIA DETAILS MALLON GIA TO ARCH ALLA AFOU GINEI TO SXHMA}. The sole purpose of the network is to predict the dense room layout (see fig\ref{data_generation}d) of an masked image. We approach this task as a classification task, where each pixel of the input image can be one of the \textit{ceiling, wall, floor} classes. This network is supervised by the dense room layouts of the dataset (see fig\ref{data_generation}d) with \textit{Cross Entropy loss}. \textbf{+ EQUATION, ALLA DEN KSERW TI ALLO MPOROUME NA POUME EDW}.

==> Model.tex <==
The DR task blurs the line between image inpainting/completion and image-to-image translation.
While image completion is among the top trends in the computer vision research, its standard approach is well formulated. 
More precisely, either pre-defined shape masks (\textit{e.g.}~boxes) are used, or free form ones, to corrupt the image, and then supervise learning with the original image.
Apart from the minor mask shape difference, DR predictions are counterfactual as they seek to reconstruct occluded areas, but similar to inpainting, it needs to exploit the context of the scene to diminish it.

Image-to-image translation on the other hand adapts the entire context of an image by translating it to another domain, like photo-to-sketch, or labels-to-image \cite{lu2018image, wang2018high}.
Usually, only part of the context needs to be preserved, most usually the dominant structure.
For our DR case, the masked region needs to be infilled with the occluded context.
While this can be considered as another domain, it is nonetheless closer to the original domain that traditional image-to-image translation tasks, which means that it can be partly inferred from its surrounding context, compared to a translated one.

\textbf{Approach.}
We employ a hybrid approach taking the masked image $\im_m = \im_f \odot \bar{\obj} + \mathbf{1} \odot \obj$ as input, with $\odot$ denoting element-wise multiplication and $\mathbf{1} \in \Omega$ is an all-ones matrix.
Our model generates an output image $\hat{\im_e}$ that with is the empty representation of the original input room.
The final diminished image $\hat{\im_d}$ is then composited as $\hat{\im_d} = \im_f \odot \bar{\obj} + \hat{\im_e} \odot \obj$.

To preserve the structural reality, our approach disentangles the structure in an explicit manner, as well as the style, which gets further disentangled per structural element.
These are then re-entangled when generating the final background image $\hat{\im_e}$, in order to preserve the structure as faithfully as possible, and to generate the appearance of each structural element distinctly.
For image inpainting this is usually done implicitly within the network, even in more recent works \cite{nazeri2019edgeconnect} that seek to respect the content's structure.
For image-to-image translation, boundary information is more important, but the assumption is that the entire image is translated, and that there are no invalid regions like holes that need to be completed.

\textbf{Structure Encoding.}
We explicitly encode the scene's structure by predicting a dense layout segmentation map $\hat{\layout} \in \Omega$ splitting the panorama into $3$ structured regions.
For this we use a well established \textit{UNet} segmentation architecture \cite{ronneberger2015u}, essentially converting structure encoding into a dense classification task. 
The input to the network is $\im_m$, and it consists of 4 down-sampling and up-sampling convolutional modules joined by skip connections, and uses batch normalization and ReLU activations.
The choice of the UNet, with skip connections and $1\!\times\!1$ prediction layers offers finer segmentation results which are very important as they allow for pixel level structure decoupling.

\textbf{Surrounding Context Encoding.}
To encode the surrounding context we use an image inpainting derived architecture, which, specifically, is adapted from \cite{yu2019free}.
Its detailed architecture is depicted in Figure~\ref{fig:networks}, and relies on Gated Convolutions, which are a generalization of partial convolutions \cite{liu2018image} that integrates a learnable gating technique when selecting features.
In addition, instance normalization \cite{ulyanov2016instance} and ReLU activations are used.
Taking into account the spherical nature of our inputs, we circularly pad \cite{sun2019horizonnet} in the horizontal image direction all convolution inputs to overcome the longitudinal boundary discontinuity, and use reflection padding to simulate the singularities at the poles \cite{zioulis2021single}.
For the bottleneck we rely on repeated dilations \cite{yu2017dilated} to capture the global context more efficiently by expanding the receptive field, avoiding additional  parameters  and  preventing  immoderate  information  loss.
This inpainting-derived encoder extracts the content excluding the hole and outputs features $\mathbf{f}_e$.

\textbf{Structure-aware Decoding.}
The decoder uses a cascade of SEAN residual blocks \cite{zhu2020sean}, gated convolutions and upsample layers.
The inputs to the decoder are the predicted structure map $\hat{\layout}$, the global context features $\mathbf{f}_e$ as encoded by the surrounding context encoder, and the original -- unmasked -- image $\im_f$.
The latter offers a set of style codes $\mathbf{f}_s^i$ for each structural element $i \in \{wall, ceiling, floor\}$ as learned by a shallow ``bottleneck'' convolutional autoencoder with a label-wise average pooling output layer.
Compared to the global context $\mathbf{f}_e$, these style codes encode local features, corresponding to texture-like details.
Through the use of SEAN blocks, we re-entangle the dense global structure $\hat{\layout}$, the global surrounding context $\mathbf{f}_e$, and the local style of each structural element $\mathbf{f}_s^i$.
This way, we condition our decoder to respect the global structure while completing the translated image, and modulate the inpainted region's style with the style codes extracted for each structural element.

\textbf{Background Discriminator.}
We use a discriminator to adaptively learn the differences between the translated empty images and the corresponding ground truth ones.
More specifically, we use a global PatchGAN \cite{isola2017image} discriminator with spectral normalization \cite{miyato2018spectral}. 
Its input is either the decoded output $\hat{\im_e}$ or the empty background image $\im_e$ concatenated with the mask $\obj$ and classifies each patch of the input image as real or fake. 
Its output $\mathbf{d}$ is a score map rather than a single score, where each value corresponds to a local region of the input sample covered by its receptive field.

\begin{comment}
\begin{enumerate}
    \item img2layout translation model:
    \begin{enumerate}
        \item UNet OR HorizonNet
        \item other important details ???
    \end{enumerate}
    \item inpainting model:
    \begin{enumerate}
        \item spherical padding
        \item edge connect backbone
        \item gated
        \item Patch Discriminator
        \item instance / spectral norm
        \item other important details ???
    \end{enumerate}
    \item SEAN connection

\item \textbf{Generator model}

The network architecture of the generator is shown \textbf{Figure (X)}. The shape for the input ($\im_{f}$ concatenated with $\obj$) and the output images is 256$\times$512. Motivated by \cite{yu2019free}, gated convolutions are utilized for the layers of the encoder and the decoder to provide a learnable dynamic feature selection mechanism for each channel and at each spatial location, achieving better visual performance than vanilla convolutions. We also adopt dilated convolutions to further expand the receptive field, avoid adding additional parameters and prevent immoderate information loss. Furthermore, we use spherical padding [\textcolor{red}{\textbf{ref needed}}] and ReLU as the activation function for all convolutional layers along with instance normalization. Finally, two SEAN blocks are adopted in the decoder, that use the predicted dense segmentation map and style code, to exploit the semantic structure and the intra-class style correlation, respectively.

Taking into consideration that normalization layers are susceptible to washing way the semantic information alongside the style correlation of the semantic classes in Indoor Scenes(in our case Ceiling, Floor, Wall) motivate us to adapt SEAN block. Hence, we exploit the input dense semantic layout $\mask$ and style $\style$ as priors to condition on them the modulation parameters (\textcolor{red}{\textbf{should we define them?}}) that contribute to attaining the semantic structure and the intra-class style consistency for the hallucinated content.

More specifically, as depicted in \textbf{Figure (X)}, the input image $\im_{f}$ and the mask $\obj$, are fed to the generator to obtain features $g^{1}_{f}$. Afterwards, $g^{1}_{f}$ along with $\style$ accompanying the downscaled $\mask$, are given to $SEANblock_1$. Subsequently, the features $g^{1}_{f}$ are first normalized and thereafter are modulated using $\mask$ and $\style$ through a spatially adaptive, learned transformation. The modulated features  $\hat{g^{1}_{f}}$ are then provided to $decoderblock_{1}$. Similarly, $SEANblock_2$ is utilized before the third block of the decoder and applied in the features $g^{3}_{f}$ to produce $\hat{g^{3}_{f}}$. 

\item \textbf{Discriminator model}
    
In previous state-of-the-art models, a local discriminator is utilized along with the global to obtain semantically and locally consistent image generation in the inpainted region and improve results. Nevertheless, using a local discriminator in the case of irregular holes is not feasible due to their non-predefined shape. Consequently, we use a global PatchGAN discriminator with spectral normalization \cite{yu2019free}. It takes as input either the completed image or the ground-truth (empty) image concatenated with the mask and classifies each patch of the input image as real or fake. Its output is a score map rather than a single score, where each value corresponds to a local region of the input sample covered by its receptive field (in our implementation, 70$\times$70).


\item \textbf{Steps followed during training and tiling artifacts \textcolor{red}{TODO: place in Discussion or here?}}

The assistance of structural information in order to obtain reasonable and realistic generated images is critical for our method. In the absence of SEAN blocks from our architecture, the performance severely deteriorates and the convergence is way slower. This is expected owing to the existence of large masks in our DR setting(in some cases they exceed the $40\%$ of the total pixels), a fact that leads to large and complex regions to be painted, composed of multiple surfaces-semantic regions. This complexity is proliferated if we take into consideration the supplementary texture complicatedness.   

Furthermore, adversarial training aids at generating spatial structures, although this occurs progressively and in conjunction with the goal of texture plausibility. With the use of SEAN blocks, the generator conditions its output in the dense segmentation map which helps to generate meaningful structures from the very beginning of the training. Given that, one would expect the network to focus more on texture generation as structure hallucination is assisted by semantic aware modulation parameters. Nonetheless, at the very start tiling artifacts appear, a fact that hinders the goal of generating photorealistic image content. 

In order to tackle these shortcomings, we use Feature Matching loss in the discriminator's feature space. Apart from the training stabilization \cite{nazeri2019edgeconnect}, the loss is conditioned on features obtained by trainable layers contrary to perceptual and style loss that are extracted via a pre-trained network. In view of this, the extracted features are capable of capturing more task-specific context that the pre-trained VGG model may be unable to localize. 

    \item supervision (do we need to focus here alot?)
    \begin{enumerate}
        \item Photometric loss:
        \item perceptual
        \item style/gram
        \item adversarial
        \item Feature Matching loss
        \item spherical weighting ($L1$)

    \end{enumerate}
    \item wide model figure:
    \begin{enumerate}
        \item with actual (intermediate and input/output) images 
        \item focus on SPADE connections
        \item decide on how much details for the models will be shown
        \item losses many not be necessary
        \item potentially use corresponding math symbols with the main document
        \item annotate the img2img translation model and the generative inpainting model, as well as their bridging/fusion (SPADE)
        \item IF e2e show grad flow?
    \end{enumerate}
\end{enumerate}
\end{comment}

==> figures/application.tex <==
\begin{figure*}[!htbp]
    \centering    
    \begin{subfigure}{.19\textwidth}
    \includegraphics[width=\textwidth]{figures/ar_dr_application/original.png}
    \subcaption{}
    \end{subfigure}
    \begin{subfigure}{.19\textwidth}
    \includegraphics[width=\textwidth]{figures/ar_dr_application/ar_no_dr.png}
    \subcaption{}
    \end{subfigure}
    \begin{subfigure}{.19\textwidth}
    \includegraphics[width=\textwidth]{figures/ar_dr_application/masked.png}
    \subcaption{}
    \end{subfigure}
    \begin{subfigure}{.19\textwidth}
    \includegraphics[width=\textwidth]{figures/ar_dr_application/inpainted.png}
    \subcaption{}
    \end{subfigure}
    \begin{subfigure}{.19\textwidth}
    \includegraphics[width=\textwidth]{figures/ar_dr_application/ar.png}
    \subcaption{}
    \end{subfigure}
    \vspace{-0.35cm}
    \caption{A demonstration of our method, which levitates AR/DR applications. 
    (a) original panorama (b) augmented reality without diminished reality (c) highlighted object for removal (d) our inpainting method result (e) augmented reality with diminished reality, the result is much more natural.}
    \label{fig:application}
    \vspace{-0.35cm}
\end{figure*}

==> figures/dataset.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}{.19\textwidth}
    \includegraphics[width=\textwidth]{figures/masked_imgs.png}
    \caption{}
    \label{fig:dataset_a}
    \end{subfigure}
    \begin{subfigure}{.19\textwidth}
    \includegraphics[width=\textwidth]{figures/empty_imgs.png}
    \caption{}
    \label{fig:dataset_b}
    \end{subfigure}
    \begin{subfigure}{.19\textwidth}
    \includegraphics[width=\textwidth]{figures/augmented_imgs.png}
    \caption{}
    \label{fig:dataset_c}
    \end{subfigure}
    \begin{subfigure}{.19\textwidth}
    \includegraphics[width=\textwidth]{figures/masked_erroneous_imgs.png}
    \caption{}
    \label{fig:dataset_d}
    \end{subfigure}
    \begin{subfigure}{.19\textwidth}
    \includegraphics[width=\textwidth]{figures/masked_correct_imgs.png}
    \caption{}
    \label{fig:dataset_e}
    \end{subfigure}
    \caption{(a) original sample with highlighted object mask, (b) empty room, (c) full room with empty supervision, (d) augmented room with objects, (e) augmented room with empty supervision}
    \label{fig:dataset}
\end{figure*}

==> figures/model.tex <==
\begin{figure*}
    \centering
    %\includegraphics[width=\textwidth]{figures/network_arch_I.png}
    \vspace{-0.25cm}
    \includegraphics[width=\textwidth]{figures/model.pdf}
    \caption{
    The PanoDR model that preserves the structural reality of the scene while counterfactually inpainting it.
    The input masked image is encoded twice, once densely by the structure UNet encoder outputing a layout segmentation map, and once by the surrounding context encoder, capturing the scene's context while taking the mask into account via series gated convolutions.
    These are then combined by the structure-aware decoder with a set of per layout component style codes that are extracted by the complete input image.
    Two SEAN residual blocks ensure the structural alignment of the reconstructed background image that is supervised by low- and high-level losses, as well as an adversarial loss driven by the background image discriminator.
    The final diminished result is created via compositing the predicted and input images using the diminishing mask.
    %The framework of the proposed approach. An input image $\im_{m}$ is given to the encoder and pre-trained segmentation network to produce features $\mathbf{f}_e$ and the dense layout $\hat{\layout}$. Afterward, the style codes $\mathbf{f}_s^i$ obtained from the $\im_{f}$ along with the dense layout  are provided to the decoder to assist in the decoding. Finally, the generated image $\hat{\im_{e}}$ is composited to produce the completed image $\hat{\im_{d}}$. The detailed architectures of the Layout Segmentation network, Style Encoder, and Discriminator are omitted for brevity.
    }
    \label{fig:networks}
    \vspace{-0.25cm}
\end{figure*}
